Small-Scale Markets for Bilateral Resource Trading in the Sharing Economy

We consider a general small-scale market for agent-to-agent resource sharing, in which each agent could either be a server (seller) or a client (buyer) in each time period. In every time period, a server has a certain amount of resources that any client could consume, and randomly gets matched with a client. Our target is to maximize the resource utilization in such an agent-to-agent market, where the agents are strategic. During each transaction, the server gets money and the client gets resources. Hence, trade ratio maximization implies efficiency maximization of our system. We model the proposed market system through a Mean Field Game approach and prove the existence of the Mean Field Equilibrium, which can achieve an almost 100% trade ratio. Finally, we carry out a simulation study motivated by an agent-to-agent computing market, and a case study on a proposed photovoltaic market, and show the designed market benefits both individuals and the system as a whole.

==> 03-best_response_policy.tex <==
As we discussed in section \ref{sec:model}, the repeated decision making problem for a single agent (with a geometrically distributed lifetime) forms a discounted cost dynamic program. Unlike a traditional market, the agent plays two roles (client or server) probabilistically over its lifetime.  In each role, the agent encounters a different decision making problem, but based on its private budget that is common to both roles.  We track a generic agent just before her role (client or server) is revealed, and we will use this sampling point in the rest of the document.  However, as an agent takes an action (bids) only after her role is revealed, this is consistent with our set-up mentioned in Section~\ref{sec:model}.  Hence, we define the Bellman equation associated with the dynamic program of interest as follows:
%\begin{equation}
%\label{eq:value_function}
%\begin{aligned}
\begin{align}
&v_{\rho}(b) =p_s v_s(b) + p_c v_c(b) \nonumber\\
&=p_s \big ( \max_{x_s\in[0,\infty)}\mathbb{E}_{\rho}[\bm{1}_{\tilde{x}_c \geq x_s}(\beta v_{\rho}(b+x_s-c_{serve})\nonumber\\
&+x_s-c_{serve})+\bm{1}_{\tilde{x}_c < x_s}\beta v_{\rho}(b)] \big) \nonumber\\
&+ p_c \big ( \max_{x_c\in[0,b+s/(1+\alpha)]}\mathbb{E}_{\rho}[\bm{1}_{x_c \geq \tilde{x}_s}(\beta v_{\rho}(b+s-\tilde{x}_s\nonumber\\
&-\alpha(\tilde{x}_s-b)^+)+s-\tilde{x}_s)+\bm{1}_{x_c < \tilde{x}_s}(\beta v_{\rho}(b)-c_{lose})] \big), %\nonumber\\
\label{eq:value_function}
\end{align}
%\end{aligned}
%\end{equation}
%\textcolor{cyan} {Note that equation (\ref{eq:value_function}) evaluates the budget value of the generic agent before she reveals her role and we will use this argument through the rest of technical discussions in this paper. This does not violate our set up mentioned in Section \ref{sec:model}, an agent first reveals her role at the beginning of each time period, then makes decisions according to the private budget status.}
where $\tilde{x}_s$ and $\tilde{x}_c$ are realizations of random variables distributed according to $\rho_s$ and $\rho_c$, and $v_\rho(\cdot)$ is the value function of a generic agent, which is in turn composed of an average of $v_s(\cdot)$ and $v_c(\cdot)$ (value functions once her role is revealed).  Since each agent's role is determined exogenously at the beginning of time period, the evolution of both $v_s(\cdot)$ and $v_c(\cdot)$ depends on $v_\rho(\cdot)$ so that \eqref{eq:value_function} remains consistent. We believe that the exogenously driven role choice makes this a natural assumption.  Since the role of the agent in our context is usually determined by the external environment, the value of the currency should be determined by the underlying market and not the role one's currently playing.

%\textcolor{cyan}{As for the thoughts of including the role into the state, the agent may end up with strategically playing different roles and have different values of same budget, both of which we would like to avoid. Because the role of the agent in our context is usually determined by the external environment that is not closable and the value of the currency should be determined by the economy of the market but not the role one currently playing.}

In our model, the client is allowed to overdraw her budget with an upper limit such that the budget does not end up negative after any possible transaction, i.e. the client is allowed to choose up to the maximum value of $x_c$ subject to  $(b+s-x_c-\alpha(x_c-b)^+)$ being non-negative. A simple calculation then yields the upper limit of a client's bid as $b+s/(1+\alpha)$. Also, for both clients and servers, when a trade happens, a budget update as well as an instantaneous gain in value is induced, which captures the fact that the trade generates value both in the present and in the future.  Further, notice that the expectation of the indicator functions in equation (\ref{eq:value_function}) can be determined using the probability of trade happening, which in turn can be calculated directly using $\rho$. Denote the c.d.f. of the assumed client and server bid distribution as $\rho_s$ and $\rho_c$, and the corresponding p.d.f./p.m.f as $p_{\tilde{x}_s}$ and $p_{\tilde{x}_c}$, respectively.  Using these we can further characterize $v_{\rho}(b)$ as follows:
%\begin{equation}
\begin{align}
%\label{eq:value_function_1}
%\begin{aligned}
%\begin{split}
&v_{\rho}(b)=\nonumber\\
&= p_s \Big ( \beta v_{\rho}(b)+\max_{x_s\in[0,\infty)}(1-\rho_c(x_s))(\beta(v_{\rho}(b+x_s-c_{serve})\nonumber\\
&-v_{\rho}(b))+x_s-c_{serve}) \Big) + p_c \Big( \max_{x_c\in[0,b+s/(1+\alpha)]}\Big[ \int_{0}^{x_c}p_{\tilde{x}_s}\nonumber\\
&(y_s)\big(\beta v_{\rho}(b+s-y_s-\alpha(y_s-b)^+)+s-y_s\big)dy_s \nonumber\\
&+(1-\rho_s(x_c))(\beta v_{\rho}(b)-c_{lose}) \Big ] \Big) \nonumber \displaybreak[0] \\
&= \beta v_{\rho}(b) + \max_{(x_s,x_c)\in\mathcal{A}(b)} \Big( \Big[  p_s(1-\rho_c(x_s))(x_s-c_{serve}) \nonumber \\
&+ p_c \big(\rho_s(x_c)(s-\mathbb{E}[\tilde{x_s}|\tilde{x}_s\leq x_c])- (1-\rho_s(x_c))c_{lose} \big) \Big] \nonumber \\
&+ \beta \Big[ p_s(1-\rho_c(x_s))\Delta v_s(b,x_s,c_{serve})\nonumber \\
&+ p_c (\int_{0}^{x_c}p_{\tilde{x}_s}(y_s)\Delta v_c(b,s,y_s,\alpha) dy_s)\Big] \Big),
\label{eq:value_function_1}
%\\
%\end{split}
%\end{aligned}
\end{align}
%\end{equation}
where\\
$\mathcal{A}(b)$ is the two dimensional bid space $\mathbb{R}_+ \times [0,b+s/(1+\alpha)],$ \\
$\Delta v_s(b,x_s,c_{serve}) = v_{\rho}(b+x_s-c_{serve}) -v_{\rho}(b),$ and \\
$\Delta v_c(b,s,y_s,\alpha) = v_{\rho}(b+s-y_s-\alpha(y_s-b)^+)-v_{\rho}(b).$ Note that the latter two functions account for the change in value with a trade for a server and a client, respectively. Then, the space of possible value functions is
\begin{equation*}
\mathcal{V}=\braces{f:(\mathbb{R}_+\rightarrow \mathbb{R}):\|f\|_\infty<\infty}=L_\infty.
\end{equation*}
Define the Bellman operator $T_\rho$ on $L_\infty$ as below:\\
%\begin{equation} \label{bell_op}
%\begin{aligned}
\begin{align}
&(T_\rho f)(b)= \beta f(b) + \max_{(x_s,x_c)\in\mathcal{A}(b)} \bigg( \Big(  p_s(1-\rho_c(x_s))(x_s \notag \\
&-c_{serve}) + p_c\big(\rho_s(x_c)(s-\mathbb{E}[\tilde{x}_s|\tilde{x}_s\leq x_c])- (1 \notag \displaybreak[0]\\
&-\rho_s(x_c))c_{lose} \big) \Big) + \beta \Big( p_s(1-\rho_c(x_s))\Delta f_s(b,x_s,c_{serve}) \notag \\
&+ p_c (\int_{0}^{x_c}p_{\tilde{x}_s}(y_s)\Delta f_c(b,s,y_s,\alpha) dy_s)\Big) \bigg)
\label{bell_op}
%\\
%\end{aligned}
%\end{equation}
\end{align}
where
%$\mathcal{A}(x)$ is the two dimensional space $[0,\infty) \times [0,b+s/(1+\alpha)]$ \\
$\Delta f_s(b,x_s,c_{serve}) = f(b+x_s-c_{serve}) -f(b),$ and
$\Delta f_c(b,s,y_s,\alpha) = f(b+s-y_s-\alpha(y_s-b)^+)-f(b).$ \\

\subsection{Properties of the Value Function}
In order to characterize the best response policy, we need to derive some useful properties of the value function $v_{\rho}$.  We start by proving the convergence of value iteration of the Bellman operator $T_\rho(\cdot)$.  This follows immediately from classical results by in \cite{hernandez1999further}, as long as we can prove the following three lemmas.

\begin{lemma}\label{lem:vi_1}
For every state $b\in \mathbb{R}_+$,
\begin{enumerate}
    \item There exists an effective bid space $\hat{\mathcal{A}}(b),$ which is compact;
    \item The reward-per-stage is lower semi-continuous in action, $(x_s,x_c)$;
    \item The function $u'(b,x_s,x_c) := \int u(s)\mathcal{Q}(ds|b,(x_s,x_c))$ is continuous in $(x_s,x_c)\in \mathcal{A}(b)$ for every function $u\in \mathcal{V}$.
\end{enumerate}
\end{lemma}
\begin{IEEEproof}
The proof of 1) follows from showing the existence of upper bounds on bids for both client and server yielding $\hat{\mathcal{A}}(b).$   The reward-per-stage in (\ref{bell_op}) is defined as  $c(b,(x_s,x_c))\triangleq p_s(1-\rho_c(x_s))(x_s-c_{serve}) + p_c \big(\rho_s(x_c)(s-\mathbb{E}[\tilde{x}_s|\tilde{x}_s\leq x_c])-(1-\rho_s(x_c))c_{lose} \big)$ and given $b,x_s,x_c$, the kernel $\mathcal{Q}$ is fully determined by $p_s,p_c,\rho$.  Details of this proof are available in Appendix \ref{app_br}.
\end{IEEEproof}

\begin{lemma}\label{lem:vi_2}
There exist constants $\xi\geq 0$ and $\eta\geq 0$ with $1\leq \eta < 1/\beta$, and a function $\omega \geq 1$ s.t. for every state $b$
\begin{enumerate}
    \item $\sup_{\mathcal{A}(b)}|c(b,(x_s,x_c))|\leq \xi \omega(b)$; and
    \item $\sup_{\mathcal{A}(b)}\int \omega(s)\mathcal{Q}(ds|b,(x_s,x_c))\leq \eta \omega(b).$
\end{enumerate}
\end{lemma}

\begin{lemma}\label{lem:vi_3}
For every state $(b)$, the function $\omega'(b,x_s,x_c):= \int \omega(s)\mathcal{Q}(ds|b,(x_s,x_c))$ is continuous in $(x_s,x_c)\in \hat{\mathcal{A}}(x)$.
\end{lemma}
\begin{IEEEproof}
Recall that since $\rho$ is the c.d.f. of some probability density function, it is absolutely continuous with respect to Lebesgue measure.  Since $c_{serve}$ and $s$ are fixed, using the continuity of $\rho$, it is straightforward to verify the results in Lemma \ref{lem:vi_2} and \ref{lem:vi_3}.
\end{IEEEproof}

\begin{theorem} (Hernandez-Lerma \cite{hernandez1999further})\label{thm:vi_converge}
Given the bid distributions (p.d.f.) of the two generic agents, $p_{\tilde{x}_s},p_{\tilde{x}_c}$, and the corresponding c.d.f. $\rho_s,\rho_c$ we have,\\
%\begin{enumerate}
%\begin{itemize}
    %\item[1)]
    1) There exists a $j\in\mathbb{N}$ such that $T_{\rho}^j:\mathcal{V}\rightarrow\mathcal{V}$ is a contraction mapping. Hence, there exists a unique $f_{\rho}^*\in\mathcal{V}$ such that $T_{\rho} f_{\rho}^*=f_{\rho}^*$, and for any $f\in\mathcal{V}$, $T^n_{\rho} f\rightarrow f_{\rho}^*$ as $n\rightarrow\infty$.\\
    %\item[2)]
    2) The fixed point $f^*_{\rho}$ of operator $T_{\rho}$ is the unique solution to the Bellman equation, i.e., $f_{\rho}^*=v_{\rho}^*$.\\
%\end{enumerate}
\end{theorem}
% \begin{IEEEproof}
% See \cite{hernandez1999further} for a detailed proof of Theorem \ref{thm:vi_converge}.
% \end{IEEEproof}

\begin{lemma} \label{lem:inc_v}
$v^*_{\rho}(b)$ is monotonically increasing in $b$.
\end{lemma}
\begin{IEEEproof}
By Theorem \ref{thm:vi_converge}, we have proved $v_{\rho}$ converges to a unique fixed point $v_{\rho}^*$ over $T_{\rho}$. Thus, it is sufficient to prove that $T_{\rho}$ maintains the assumed monotonicity. Full details of the proof are presented in Appendix \ref{app_br}.
\end{IEEEproof}

\subsection{Best Response Policy Characterization}

As discussed in Section~\ref{sec:model}, our goal is to maximize server utilization from the system perspective, which is equivalent to maximizing the expected trade ratio in the market.  Furthermore, the budget, which is defined through equation (\ref{eq:value_function}), increases through successful trade. These observations imply that we should characterize the best response policy not only from the single agent perspective, but also from the perspective of maximizing the expected trade ratio.  We will use this goal to motivate a specific family of equilibria for our problem.  We start with a few easily established facts regarding equilibrium behavior of the agents. %Before moving further, we discuss the following three facts.

\begin{fact} \label{fact1}
Given $\rho_s$, a client should never bid higher than $\bar{x}_s$, where $\bar{x}_s$ is the upper-end of the support of $\rho_s$, i.e., $\rho_s(x_s)=1\ \forall x_s\geq\bar{x}_s$ and $\rho_s(x_s)<1\ \forall x_s<\bar{x}_s$.
\end{fact}

\begin{fact} \label{fact2}
Given $\rho_c$, a server should never bid higher than $\bar{x}_c$, where $\bar{x}_c$ is the lower-end of the support of $\rho_c$, i.e., $\rho_c(x_c)=1\ \forall x_c\geq\bar{x}_c$ and $\rho_c(x_c)<1\ \forall x_c<\bar{x}_c$.
\end{fact}

\begin{fact} \label{fact3}
Given $p_{\tilde{x}_s}$, a client should never bid $x$ for $x>0$ such that $p_{\tilde{x}_s}(x)=0$ (even if support is not a connected set).
\end{fact}
%\textcolor{blue}{Does Fact 3 also hold if the support of $\rho_s$ is not connected? It seems to be true, so clarify it.}
%\textcolor{cyan}{What does 'not connected' support mean?}

These three facts hold since the violation each of them yields a non-positive payoff to a generic agent. Thus, we claim that if an equilibrium exists, which we will discuss in section \ref{sec:mfe}, then in each equilibrium, $\bar{x}_s=\bar{x}_c$.

Assuming that the facts above hold, we then show that for the best system performance a certain simpler class of bidding functions suffice.
\begin{lemma} \label{lem:single_price}
All servers bidding the same price within the clients' affordable range maximizes the expected trade ratio.
\end{lemma}
\begin{IEEEproof}
The proof follows from by comparing the trade ratios between the scenarios in which the server places multiple bids or a single bid.  Using the three facts above, the corresponding client bid distributions can be further characterized.  Full details are available in Appendix \ref{app_br}.
\end{IEEEproof}

Motivated by Lemma~\ref{lem:single_price}, we characterize the best response policy by initializing the belief of server's bid distribution to be $p_{\tilde{x}_s}(k)=1$ for some fixed $k$, i.e. all servers bid the same price $k$.  For non-trivial behavior $k\geq c_{serve}$, but $k$ can be higher than $s$, though not by much, i.e. $s-k\geq c_{lose}$, otherwise, the trade will become worthless; see section \ref{sec:sim} for the latter.

\subsubsection{Client's Best Response}

Given the belief of the single price $k$ that all servers bid, the value function of clients from (\ref{eq:value_function}) becomes
\begin{equation}
\begin{aligned}
& v_c(b)=\max_{x_c\in[0,b+s/(1+\alpha)]} \Big( \bm{1}_{x_c \geq k}(\beta(v_{\rho}(b+s-k \\
&\quad -\alpha(k-b)^+))+s-k)+\bm{1}_{x_c < k}(\beta v_{\rho}(b)-c_{lose}) \Big ) \\
\end{aligned}
\end{equation}
By Facts \ref{fact1} and \ref{fact3}, we conclude that the client will bid either $0$ or $k.$ If a client bids $k$, the trade will happen w.p. $1$, and will fail otherwise.  We define the following useful terms: \\
$v_{c\_win}(b) = \beta(v_{\rho}^*(b+s-k-\alpha(k-b)^+))+s-k$, \\
$v_{c\_lose}(b) = \beta v_{\rho}^*(b)-c_{lose}$,
$b_{c\_win} = b+s-k-\alpha(k-b)^+$, and
$b_{c\_lose}= b$.

Since the budget can never go negative, we have an upper limit on a client's bid of $b+s/(1+\alpha)$.  If $k$ lies out of this range, the client will simply bid $0$.  Now, from Lemma \ref{lem:inc_v}, $b_{c\_win} \geq b_{c\_lose}$ i.e. $b\geq ((1+\alpha)k-s)/\alpha=k-\frac{s-k}{\alpha}$ implies that if $v_{c\_win}(b) \geq v_{c\_lose}(b)$, then the client should bid $k$.  Thus, we have a lower bound on the bid as $0$, and the upper bound as $k$. The exact bidding strategy depends on the relationship between $v_{c\_win}(b)$ and $v_{c\_lose}(b)$.  A summary of the best responses of a client with budget $b$ is:
\begin{equation} \label{client_br}
x_c^*=  \\
\begin{aligned}
\begin{cases}
0 & b\in[0,k-\frac{s}{1+\alpha}) \\
0 \text{ if } v_{c\_win}(b) \leq v_{c\_lose}(b) & b\in[k-\frac{s}{1+\alpha},k-\frac{s-k}{\alpha}] \\
k \text{ if } v_{c\_win}(b) \geq v_{c\_lose}(b) & b\in[k-\frac{s}{1+\alpha},k-\frac{s-k}{\alpha}] \\
k & b\in(\frac{(1+\alpha)k-s}{\alpha}, \infty) \\
\end{cases}
\end{aligned}
\end{equation}

Note that when $k<s/(1+\alpha)$, all clients will bid $k,$ which is an extreme case of a ``cheap resource."  It implies the price one needs to pay is too low, as compared to the gain from the trade.  We further characterize the best response function $\theta_{c,\rho}(b)$ in the following Lemma.
\begin{lemma} \label{lem:finite_pieces}
$\theta_{c,\rho}(b)$ has finite pieces of continuous constant intervals on $[0,k-\frac{s-k}{\alpha}]$.
\end{lemma}
\begin{IEEEproof}
The proof follows by showing the difference $v_{c\_win}(b)-v_{c\_lose}(b)$ is of bounded total variation.  Full details are available in Appendix \ref{app_br}.
\end{IEEEproof}



\subsubsection{Server's Best Response}

Given the client's best response function, we observe that under certain circumstances, the client will bid either $0$ or $k$ based on her private state.  By Facts \ref{fact2} and \ref{fact3}, we conclude that the server will again bid either $0$ or $k$.  We can refine the server's belief about the client's bid distribution as $p_{\tilde{x}_c}=(z,1-z)$, where $z=\mathbb{P}(\tilde{x}_c=0)$.  Then
\begin{equation*}
v_s(b) = (1-z)(\beta v_{\rho}(b+x_s-c_{serve})+x_s-c_{serve}) + z \beta v_{\rho}(b).
\end{equation*}
By Lemma \ref{lem:inc_v}, for $\forall b\in\mathbb{R}_+$, we have $v_s(b)$ is monotonically increasing in $x_s$, when $x_s\leq k$.  Hence, all servers will bid $k$.

%Given $k$, the coupling of the client's and server's best response function implies our market system may admit an equilibrium over the simple belief $p_0$. We will prove the corresponding Mean Field Equilibrium (MFE) indeed exist in section \ref{sec:mfe}.

Given a feasible $k$ (which we refer to as a ``unified price'' for both clients and servers), the discussion above lends credence to the existence of an equilibrium over the simple set of beliefs given by $z$.  We will prove that such  Mean Field Equilibrium (MFE) indeed exists in section \ref{sec:mfe}.



















